OkraLong: A Flexible Retrieval-Augmented Framework for Long-Text Query Processing

Large Language Models (LLMs) encounter challenges in efficiently processing long-text queries, as seen in applications like enterprise document analysis and financial report comprehension. While conventional solutions employ long-context processing or Retrieval-Augmented Generation (RAG), they suffer from prohibitive input expenses or incomplete information. Recent advancements adopt context compression and dynamic retrieval loops, but still sacrifice critical details or incur iterative costs. To address these limitations, we propose OkraLong, a novel framework that flexibly optimizes the entire processing workflow. Unlike prior static or coarse-grained adaptive strategies, OkraLong adopts fine-grained orchestration through three synergistic components: analyzer, organizer and executor. The analyzer characterizes the task states, which guide the organizer in dynamically scheduling the workflow. The executor carries out the execution and generates the final answer. Experimental results demonstrate that OkraLong not only enhances answer accuracy but also achieves cost-effectiveness across a variety of datasets.

==> formulation.tex <==
\section{Preliminary}
\subsection{Problem Definition}

Given a long-form text corpus \( D \), the processing system $\mathcal{P}$ is responsible to process the text and generate the answer \( a \) for each query \( q \): 
\begin{equation}
a = \mathcal{P}(q,D)
\label{eq:1}
\end{equation}

In practical settings, the long-text understanding task should be formalized as a comprehensive multi-objective optimization problem with the following requirement: 
Provide high-quality responding answers for varied queries; maintain a low financial cost; keep acceptable latency overhead.


% Thus, due to  simplification and the clearity, we define the good put to comprehensive measure the performance of a processsing pipeline:
% \begin{equation}
% \text{GoodPut} = \text{Acc} - \ \lambda_1 \cdot \text{cost} - \lambda_2 \cdot \text{latency}
% \label{eq:2}
% \end{equation}
% where \( \lambda_i \) denote preference-related weights for the penalty of cost and latency.
% And the optimization target can be formalized as: given q, D:
% \begin{equation}
% \max_{\mathcal{P}} \text{GoodPut}(\mathcal{P},q,D)
% \end{equation}
 

\subsection{Method Formulation}
Conventional RAG frameworks employ static retriever that select top-\( k \) text chunks through relevant matching and send the chunks to the LLM for answering.
\begin{equation}
C_{\text{base}} = \{c_1, ..., c_k\} = \texttt{Ret}(q,D)
\label{eq:2}
\end{equation}
\begin{equation}
a = \texttt{LLM}(q,C_{\text{base}})
\label{eq:2}
\end{equation}
where $c_i$ means the segmented text chunks and the \texttt{Ret} means the deployed retriever.


Advanced RAG variants introduce conditional retrieval based on LLMs feedback:
\begin{equation}
C_{\text{adv},t} = \begin{cases} 
\emptyset  &\text{if } \varGamma(a_{t-1},q) \\
\texttt{Ret}(\varGamma(a_{t-1},q),D) & \text{otherwise}
\end{cases}
\end{equation}
\begin{equation}
a_{t}=LLM(C_{\text{adv},t},q)
\label{eq:3}
\end{equation}
where \( \texttt{Check} \) evaluates partial response \( a_{\text{init}} \)'s confidence.

Our framework OkraLong is designed as a more flexible framework.
A task analyzer determines task states \( \tau \in \mathcal{T} \) which are then utilized to get the running plans and the configurations:
\begin{equation}
\{\theta, \psi, \phi\}= \Omega(\texttt{Analyzer}(q,D))
\label{eq:4}
\end{equation}
Subsequently, the system adapts retrieval parameters \( \theta \), chunking strategy \( \psi \), and generation policy \( \phi \) through task-aware modulation:
\begin{equation}
\{\theta, \psi, \phi\} = \Omega(\tau, \text{env})
\label{eq:5}
\end{equation}
where \( \text{env} \) denotes runtime constraints including computational budget \( b \) and latency threshold \( l \).



